Learning from Label Proportions: Bootstrapping Supervised Learners via Belief Propagation

Learning from Label Proportions (LLP) is a learning problem where only aggregate level labels are available for groups of instances, called bags, during training, and the aim is to get the best performance at the instance-level on the test data. This setting arises in domains like advertising and medicine due to privacy considerations. We propose a novel algorithmic framework for this problem that iteratively performs two main steps. For the first step (Pseudo Labeling) in every iteration, we define a Gibbs distribution over binary instance labels that incorporates a) covariate information through the constraint that instances with similar covariates should have similar labels and b) the bag level aggregated label. We then use Belief Propagation (BP) to marginalize the Gibbs distribution to obtain pseudo labels. In the second step (Embedding Refinement), we use the pseudo labels to provide supervision for a learner that yields a better embedding. Further, we iterate on the two steps again by using the second step's embeddings as new covariates for the next iteration. In the final iteration, a classifier is trained using the pseudo labels. Our algorithm displays strong gains against several SOTA baselines (up to 15%) for the LLP Binary Classification problem on various dataset types - tabular and Image. We achieve these improvements with minimal computational overhead above standard supervised learning due to Belief Propagation, for large bag sizes, even for a million samples.

==> Motivation.tex <==
\section{Motivation}
The table below highlights the performance obtained on using oracle labels for instances with different levels of noise added to the labels.
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Noise & Downstream AUC & Val. Contrastive loss & Avg. Pos-Neg Similarity Diff & Optimizer for embed. learning \\ \hline
0.0 & 0.7973 & 12.76 & 0.2180 & Adam \\ \hline
0.05 & 0.8001 & 12.75 & 0.2174 & SGD \\ \hline 
0.10 & 0.8019 & 12.75 & 0.2068 & SGD \\ \hline
0.15 & 0.7996 & 12.77 & 0.1901 & SGD \\ \hline
0.20 & 0.7973 & 12.80 & 0.1628 & SGD \\ \hline
0.25 & 0.7902 & 12.86 & 0.1304 & SGD \\ \hline
0.30 & 0.7859 & 12.93 & 0.0830 & SGD \\ \hline
\end{tabular}%
}
\caption{Oracle Contrastive performance on feature bags of size 32. Baseline DLLP AUC: 0.7900 with SGD, 0.7815 with Adam}
\label{tab:oracle}
\end{table}

It has been observed that as the complexity of the pooling methods increases the quality of the instance embeddings learnt, that are to be extracted from before the pooling layer degrades. It can be understood to be due to the higher computational power the complex pooling layer provides, thus learning more complex correlations between the instances within a bag. Hence as these correlations are captured by the pooling layer, even if the instance embeddings learnt are subpar, the pooling layer takes care of the learning. whereas for simple pooling techniques like mean pooling, the learning must be ensured in the instance embeddings itself as the pooling layer can only capture limited patterns between the instances. 

\textbf{TABLE TBA}

So using a more complicated pooling method to learn bag embeddings might not be the right way ahead. A better bag level evaluation performance does not necessarily translate to better instance level evaluation performance which is our eventual task. So we must look at ways to actually provide an instance level signal to improve our embedding quality.


==> datasets.tex <==
\begin{itemize}[leftmargin=10pt]
\item UCI Tabular Datasets
\begin{itemize}[leftmargin=10pt]
    \item \textbf{Adult Income} \citep{Dua:2019} \cite{kohavi1996scaling}:
     Classification task is to predict whether a person makes over \$50K a year based on the provided census data of 14 features. We split the data into 90-10 train-test split and then further use 10\% of the training data as a hold-out validation set is in the literature \citep{friedman2001greedy}
    \item \textbf{Bank Marketing} \citep{Dua:2019} \cite{moro2011using}: 
    The task here it to predict if the client will subscribe a term deposit from 16 features. We use the original \cite{moro2014data} method of splitting the customers into $\frac{2}{3}$-$\frac{1}{3}$ train-test split and then further using $\frac{1}{3}$ of the training set as a hold-out validation set.

\end{itemize}
\item Large Tabular Data
\begin{itemize}[leftmargin=10pt]
    \item \textbf{Criteo}: One-week data from CriteoLabs for click-through-rate (CTR) prediction summing up to 45M samples with 39 features each. We sample non-overlapping sets of 1 million, 200k and 250k points to form our train, validation and test datasets respectively. 
    This dataset is especially important for its scale and difficulty.
\end{itemize}
\item Image Data
\begin{itemize}[leftmargin=10pt]
    \item \textbf{CIFAR-10}: 60k images each of size 32$\times$32$\times$3. These images belong to 10 classes, each containing 6k images. We use this predefined test-set containing 10k images as our test data, and randomly sample 10\% images from the predefined train-set (50k images) to form our validation data. We also binarize this data to form 2 different variants of CIFAR-10 inspired by \cite{busa2023easy}
    \begin{itemize}[leftmargin=10pt]
        \item \textbf{CIFAR-B}: We assign label \textit{1} to all \textit{Machine} classes (0,1,8,9) and label \textit{0} to all \textit{Animal} classes (2,3,4,5,6,7). In this dataset, 40\% of all instances belong to the positive class. 
        \item \textbf{CIFAR-S}: All instances belonging to the class \textit{Ship} are assigned label \textit{1} and all other instances are assigned label \textit{0}. This dataset has 10\% positive instances and is more skewed.
    \end{itemize}
\end{itemize}\end{itemize}


